Avoid Forgetting by Preserving Global Knowledge Gradients in Federated Learning with Non-IID Data

The inevitable presence of data heterogeneity has made federated learning very challenging. There are numerous methods to deal with this issue, such as local regularization, better model fusion techniques, and data sharing. Though effective, they lack a deep understanding of how data heterogeneity can affect the global decision boundary. In this paper, we bridge this gap by performing an experimental analysis of the learned decision boundary using a toy example. Our observations are surprising: (1) we find that the existing methods suffer from forgetting and clients forget the global decision boundary and only learn the perfect local one, and (2) this happens regardless of the initial weights, and clients forget the global decision boundary even starting from pre-trained optimal weights. In this paper, we present FedProj, a federated learning framework that robustly learns the global decision boundary and avoids its forgetting during local training. To achieve better ensemble knowledge fusion, we design a novel server-side ensemble knowledge transfer loss to further calibrate the learned global decision boundary. To alleviate the issue of learned global decision boundary forgetting, we further propose leveraging an episodic memory of average ensemble logits on a public unlabeled dataset to regulate the gradient updates at each step of local training. Experimental results demonstrate that FedProj outperforms state-of-the-art methods by a large margin.

==> algorithms.tex <==
\section{Algorithms}


% \begin{algorithm}
% \caption{Federated Learning with FedProj and Knowledge Distillation}
% \label{alg:FedProjKD}
% \begin{algorithmic}[1]

% \REQUIRE number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epochs ($E$), local batch size ($B$), learning rate ($\eta$), temperature ($T$), distillation learning rate ($\eta_d$), distillation epochs ($E_d$), regularization coefficient ($\gamma$).

% \STATE \textbf{Server Executes:}
% \STATE Initialize global model $\btheta_g^0$
% \FOR {$t = 0, 1, \ldots, T-1$}
%     \STATE Sample $m = \max(C \cdot N,1)$ clients $S_t$
%     \FOR {$k \in S_t$ \textbf{in parallel}}
%         \STATE $\btheta^{t+1}_{k} \gets \mathtt{ClientUpdate}(k; \btheta^t_{g})$
%     \ENDFOR

%     \STATE \textbf{FedAvg:}  
%     \STATE
%     \[
%     \btheta^{t+1}_g = \sum_{k \in S_t} \frac{|D_k|}{\sum_{j \in S_t} |D_j|} \btheta^{t+1}_k
%     \]
%     \STATE Evaluate $\btheta_g^{t+1}$ on test set.

%     \STATE \textbf{Logits Averaging:}  
%     \STATE
%     \[
%     \mathcal{Z}_{\text{teacher}} = \frac{1}{|S_t|} \sum_{k \in S_t} f_k(\mathcal{D}_{\text{public}}; \btheta_k^{t+1})
%     \]

%     \STATE \textbf{Global Model KD:}
%     \FOR {$e = 1, \ldots, E_d$}
%         \FOR {each batch $(\mathbf{x}, \mathbf{z}_{\text{teacher}}) \in \mathcal{D}_{\text{public}}$}
%             \STATE Compute student logits:
%             \STATE
%             \[
%             \mathcal{Z}_{\text{student}} = f_g(\mathbf{x}; \btheta_g)
%             \]
%             \STATE Compute loss:
%             \STATE
%             \[
%             \mathcal{L}_{\text{KD}} = T^2 \cdot \text{KL}(\sigma(\mathcal{Z}_{\text{student}} / T), \sigma(\mathcal{Z}_{\text{teacher}} / T))
%             \]
%             \STATE
%             \[
%             \mathcal{L}_{\text{reg}} = \gamma \sum_{i} \|\btheta_g^{(i)} - \btheta_g^{(i,0)}\|^2
%             \]
%             \STATE Update model:
%             \STATE
%             \[
%             \btheta_g \gets \btheta_g - \eta_d \nabla_{\btheta_g} (\mathcal{L}_{\text{KD}} + \mathcal{L}_{\text{reg}})
%             \]
%         \ENDFOR
%     \ENDFOR
% \ENDFOR

% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{ClientUpdate with FedProj and Knowledge Distillation}
% \label{alg:ClientFedProjKD}
% \begin{algorithmic}[1]
% \REQUIRE Local dataset $\mathcal{D}_k$, learning rate $\eta$, temperature $T$, distillation dataset $\mathcal{D}_{\text{public}}$, regularization $\gamma$.
% \STATE Initialize local model $\btheta_k$.
% \FOR{$e = 1$ to $E$} 
%     \FOR{each mini-batch $(\mathbf{x}, \mathbf{y}) \sim \mathcal{D}_k$} 
%         \STATE Compute local logits: $\mathcal{Z}_{\text{local}} = f_k(\mathbf{x}; \btheta_k)$
%         \STATE Compute supervised loss: $\mathcal{L}_{\text{sup}} = \ell(\mathcal{Z}_{\text{local}}, \mathbf{y})$
%         \STATE Sample public batch: $(\mathbf{x}_t, \mathcal{Z}_{t}) \sim \mathcal{D}_{\text{public}}$
%         \STATE Compute student logits:  \\$\mathcal{Z}_{\text{student}} = f_k(\mathbf{x}_t; \btheta_k)$
%         \STATE Compute KD loss:
%         \[
%         \mathcal{L}_{\text{KD}} = T^2 \cdot \text{KL}(\sigma(\mathcal{Z}_{\text{student}} / T), \sigma(\mathcal{Z}_{t} / T))
%         \]
%         \STATE Compute gradients:  
%         \[
%         g_{\text{new}} = \nabla_{\btheta_k} \mathcal{L}_{\text{sup}}, \quad g_{\text{glob}} = \nabla_{\btheta_k} \mathcal{L}_{\text{KD}}
%         \]
%         \STATE Compute projected gradient:  
%         \[
%         g_{\text{proj}} = g_{\text{new}} - \frac{\langle g_{\text{new}}, g_{\text{glob}} \rangle}{\| g_{\text{glob}} \|^2 + \epsilon} g_{\text{glob}}
%         \]
%         \STATE Update model parameters: 
%         \[
%         \btheta_k \gets \btheta_k - \eta g_{\text{proj}}
%         \]
%     \ENDFOR
% \ENDFOR
% \RETURN $\btheta_k$
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{Federated Learning}
% \label{alg:FedAvg}

% % \DontPrintSemicolon
% % \SetCommentSty{mycommfont}
% % \SetAlgoLined
% % \SetKwInOut{Req}{Require}
% % \SetKwFunction{FClient}{ClientUpdate}
% % \SetKwProg{Fn}{}{:}{}

% \begin{algorithmic}[1]
% \REQUIRE number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
% %\SetKwProg{Fn}{Server Executes}{:}{}
% \STATE \textbf{Server Executes:}
% \STATE Initialize the server model with $\btheta_g^0$ \;
% \FOR {each round $t = 0, 1, \ldots, T-1$}
% \STATE $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
% \STATE $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
% \FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% \STATE $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
% %$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% \ENDFOR
% \STATE $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
% \ENDFOR
% \vspace{1mm}
% \FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
% \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
% \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k^{train}$ into batches of Size $B$})\;
% \FOR {each local epoch $ \in \{1, \ldots, E\}$}
% \FOR {each batch $\mathbf{b} \in \mathcal{B}$}
% \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} \ell(f_k(\bx; \btheta^{t}_k), y)$\;
% \ENDFOR
% \ENDFOR
% \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
% \ENDFUNCTION
% % \Fn{\FClient{$k, \btheta^t_{g}$}}{
% %     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
% %     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
% %     \For {each local epoch $i = 1, \dots, E$} {
% %         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
% %             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
% %         }
% %     }
% %     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
% %     \KwRet $\btheta^{t+1}_{k}$\;
% % }
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{Federated Learning with FedProj}
% \label{alg:FedProj}

% \begin{algorithmic}[1]
% \REQUIRE number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epochs ($E$), local batch size ($B$), learning rate ($\eta$), temperature ($T$), memory batch size ($M$).
% \STATE \textbf{Server Executes:}
% \STATE Initialize the server model with $\btheta_g^0$ \;
% \FOR {each round $t = 0, 1, \ldots, T-1$}
% \STATE $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
% \STATE $S_t \leftarrow $(random set of $m$ clients) \; 
% \FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% \STATE $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
% \ENDFOR
% \STATE $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
% \STATE Perform knowledge distillation to update $\btheta^{t+1}_{g}$
% \ENDFOR
% \vspace{1mm}
% \FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
% \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
% \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k^{train}$ into batches of Size $B$})\;
% \FOR {each local epoch $ \in \{1, \ldots, E\}$}
% \FOR {each batch $\mathbf{b} \in \mathcal{B}$}
% \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} \ell(f_k(\bx; \btheta^{t}_k), y)$\;
% \ENDFOR
% \ENDFOR
% \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
% \ENDFUNCTION
% \end{algorithmic}
% \end{algorithm}



% \begin{algorithm}[H]
% \caption{FedAvg}
% \label{alg:FedAvg}

% % \DontPrintSemicolon
% % \SetCommentSty{mycommfont}
% % \SetAlgoLined
% % \SetKwInOut{Req}{Require}
% % \SetKwFunction{FClient}{ClientUpdate}
% % \SetKwProg{Fn}{}{:}{}

% \begin{algorithmic}[1]
% \STATE \textbf{Require:} number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
% %\SetKwProg{Fn}{Server Executes}{:}{}
% \STATE \textbf{Server Executes:}
% \STATE $\quad$ Initialize the server model with $\btheta_g^0$ \;
% \FOR {each round $t = 0, 1, \dots, T-1$}
% \STATE $\quad$ $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
% \STATE $\quad$ $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
% $\quad$ \FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% \STATE $\quad$ $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
% %$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% \ENDFOR
% \STATE $\quad$ $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
% \ENDFOR
% \vspace{1mm}
% \FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
% \STATE H
% \ENDFUNCTION
% % \Fn{\FClient{$k, \btheta^t_{g}$}}{
% %     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
% %     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
% %     \For {each local epoch $i = 1, \dots, E$} {
% %         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
% %             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
% %         }
% %     }
% %     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
% %     \KwRet $\btheta^{t+1}_{k}$\;
% % }
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{FedProx}
% \label{alg:FedProx}

% \DontPrintSemicolon
% \SetCommentSty{mycommfont}
% \SetAlgoLined
% \SetKwInOut{Req}{Require}
% \SetKwFunction{FClient}{ClientUpdate}

% \Req{number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), 
% local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$), FedProx parameter ($\mu$)\;}
% \SetKwProg{Fn}{Server Executes}{:}{}
% \Fn{}{
% Initialize the server model with $\theta_g^0$ \;
% \For {each round $t = 0, 1, \dots, T-1$} {
%  $m \leftarrow {\rm{max}}(C \cdot N,1)$\;
%  $S_t \leftarrow $(random set of m clients)\; %\tcp*{set of $m$ available clients}
% \For  {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% { 
% $\theta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \theta^t_{g} )$ \; 
% }

% $\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% }
% }
% %\Indm
% \SetKwProg{Fn}{}{:}{}
% \Fn{\FClient{$k, \theta^t_{g}$}}{
%      $\theta^{t}_k \leftarrow \theta^t_{g}$\;
%      $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
%     \For {each local epoch $i = 1, \dots, E$} {
%         \For {each batch $\mathbf{b} \in \mathcal{B}$} 
%         {
%              $\theta^{t+1}_k \leftarrow \argmin_{\theta_k} \mathbb{E} \left[ f(\theta_k; \mathbf{b}) \right] + \frac{\mu}{2} ||\theta_k - \theta^t_k||^2$\;
%         }
%     }
%     $\theta^{t+1}_k \leftarrow \theta^{t}_k$\;
%     \KwRet $\theta^{t+1}_{k}$\;
% }
% \end{algorithm}



==> macros.tex <==

\usepackage[mathscr]{euscript}
\usepackage{accents}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}

% Copied from mathrsfs.sty
\DeclareSymbolFont{rsfs}{U}{rsfs}{m}{n}
\DeclareSymbolFontAlphabet{\mathscrsfs}{rsfs}

% Probability
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\text{Var}}
\newcommand{\Cov}{\text{Cov}}
%\newcommand{\cN}{\mathcal{N}}
\newcommand{\Expect}{{\mathbb E}}

% Sets
%\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\S}{\mathbb{S}}

\def\reals{{\mathbb R}}
\def\ball{{\mathsf B}}

% Variables
\newcommand{\eps}{\varepsilon} 
\newcommand{\vphi}{\varphi}
\def\id{{\mathbf I}}


% Math
\renewcommand{\d}{\textup{d}}
\renewcommand{\l}{\vert}
\newcommand{\dl}{\Vert}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
%\newcommand{\sign}{\text{sign}}
\newcommand{\diag}{\text{diag}}
%\newcommand{\tr}{\text{tr}}
\newcommand{\op}{}
\newcommand{\ones}{\bm{1}}
\newcommand{\what}{\widehat}
\newcommand{\grad}{\nabla}
\def\sT{{\mathsf T}}
\def\bzero{{\boldsymbol 0}}


\def\tu{\tilde{u}}
\def\tg{\tilde{g}}

% Bold symbols
\def\bA{{\boldsymbol A}}
\def\bB{{\boldsymbol B}}
\def\bC{{\boldsymbol C}}
\def\bD{{\boldsymbol D}}
\def\bE{{\boldsymbol E}}
\def\bF{{\boldsymbol F}}
\def\bG{{\boldsymbol G}}

\def\bH{{\boldsymbol H}}
\def\bJ{{\boldsymbol J}}
\def\bK{{\boldsymbol K}}
\def\bL{{\boldsymbol L}}
\def\bM{{\boldsymbol M}}
\def\bO{{\boldsymbol O}}
\def\bP{{\boldsymbol P}}
\def\bQ{{\boldsymbol Q}}
\def\bR{{\boldsymbol R}}
\def\bS{{\boldsymbol S}}
\def\bT{{\boldsymbol T}}
\def\bU{{\boldsymbol U}}
\def\bV{{\boldsymbol V}}
\def\bW{{\boldsymbol W}}
\def\bX{{\boldsymbol X}}
\def\bY{{\boldsymbol Y}}
\def\bZ{{\boldsymbol Z}}

\def\tZ{\tilde{Z}}

\def\tbU{\tilde{\boldsymbol U}}
\def\tbZ{\tilde{\boldsymbol Z}}
\def\tbg{\tilde{\boldsymbol g}}

\def\ba{{\boldsymbol a}}
\def\bb{{\boldsymbol b}}
\def\be{{\boldsymbol e}}
\def\boldf{{\boldsymbol f}}
\def\bg{{\boldsymbol g}}
\def\bh{{\boldsymbol h}}
\def\bi{{\boldsymbol i}}
\def\bj{{\boldsymbol j}}
\def\bk{{\boldsymbol k}}
\def\bt{{\boldsymbol t}}
\def\bu{{\boldsymbol u}}
\def\bv{{\boldsymbol v}}
\def\bw{{\boldsymbol w}}
\def\bx{{\boldsymbol x}}
\def\by{{\boldsymbol y}}
\def\bz{{\boldsymbol z}}

\def\bbeta{{\boldsymbol \beta}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol \eps}}
\def\blambda{{\boldsymbol \lambda}}
\def\bpsi{{\boldsymbol \psi}}
\def\bphi{{\boldsymbol \phi}}
\def\hbtheta{\hat{\boldsymbol \theta}}
\def\hbbeta{\widehat{\boldsymbol \beta}}
\def\hbeta{\widehat{\beta}}
\def\btheta{{\boldsymbol \theta}}
\def\bvphi{{\boldsymbol \vphi}}
\def\bxi{{\boldsymbol \xi}}

\def\bDelta{{\boldsymbol \Delta}}
\def\bLambda{{\boldsymbol \Lambda}}
\def\bPsi{{\boldsymbol \Psi}}
\def\bPhi{{\boldsymbol \Phi}}
\def\bSigma{{\boldsymbol \Sigma}}
\def\bTheta{{\boldsymbol \Theta}}

\def\bfzero{{\boldsymbol 0}}
\def\bfone{{\boldsymbol 1}}



% Symbols with hat
\def\hba{{\widehat {\boldsymbol a}}}
\def\hf{{\widehat f}}
\def\tcT{\widetilde{\mathcal T}}
\def\tK{\widetilde{K}}




% rm symbols
\def\spn{{\rm span}}
\def\supp{{\rm supp}}
\def\Easy{{\rm E}}
\def\Hard{{\rm H}}
\def\post{{\rm post}}
\def\pre{{\rm pre}}
\def\Rot{{\rm Rot}}
\def\Sft{{\rm Sft}}
\def\endd{{\rm end}}
\def\KR{{\rm KR}}
\def\bbHe{{\rm He}}
\def\sk{{\rm sk}}
\def\de{{\rm d}}
\def\He{{\rm He}}
\def\Trace{{\trace}}
\def\lin{{\rm lin}}
\def\res{{\rm res}}
\def\degzero{{\rm deg0}}
\def\degone{{\rm deg1}}
\def\Poly{{\rm Poly}}
\def\Poly{{\rm Poly}}
\def\Coeff{{\rm Coeff}}
\def\de{{\rm d}}
\def\Unif{{\rm Unif}}
\def\He{{\rm He}}
\def\lin{{\rm lin}}
\def\res{{\rm res}}
\def\RF{{\rm RF}}
\def\NT{{\rm NT}}
\def\NF{{\rm NF}}
\def\Cyc{{\rm Cyc}}
\def\RC{{\rm RC}}
\def\kernel{\rm Ker}
\def\image{{\rm Im}}
\def\Easy{{\rm E}}
\def\Hard{{\rm H}}
\def\post{{\rm post}}
\def\pre{{\rm pre}}
\def\Rot{{\rm Rot}}
\def\Sft{{\rm Sft}}
\def\ddiag{{\rm ddiag}}
\def\KR{{\rm KR}}
\def\RR{{\rm RR}}
\def\bbHe{{\rm He}}
\def\eff{{\rm eff}}

\def\spn{{\rm span}}


%mathcal symbols
\def\cV{{\mathcal V}}
\def\cG{{\mathcal G}}
\def\cO{{\mathcal O}}
\def\cP{{\mathcal P}}
\def\cW{{\mathcal W}}
\def\cT{{\mathcal T}}
\def\cC{{\mathcal C}}
\def\cQ{{\mathcal Q}}
\def\cL{{\mathcal L}}
\def\cF{{\mathcal F}}
\def\cE{{\mathcal E}}
\def\cS{{\mathcal S}}
\def\cI{{\mathcal I}}
\def\cV{{\mathcal V}}
\def\cG{{\mathcal G}}
\def\cO{{\mathcal O}}
\def\cP{{\mathcal P}}
\def\cW{{\mathcal W}}
\def\cT{{\mathcal T}}
\def\cH{{\mathcal H}}
\def\cA{{\mathcal A}}



%mathbb mathsf sf symbols
\def\K{{\mathbb K}}
\def\H{{\mathbb H}}
\def\T{{\mathbb T}}
\def\bbV{{\mathbb V}}
\def\W{{\mathbb W}}
\def\sM{{\mathsf M}}
\def\sW{{\mathsf W}}
\def\Unif{{\sf Unif}}
\def\normal{{\sf N}}
\def\proj{{\mathsf P}}
\def\ik{{\mathsf k}}
\def\il{{\mathsf l}}
\def\sM{{\sf M}}
\def\RKHS{{\sf RKHS}}
\def\RF{{\sf RF}}
\def\NT{{\sf NT}}
\def\NN{{\sf NN}}
\def\reals{{\mathbb R}}
\def\integers{{\mathbb Z}}
\def\naturals{{\mathbb N}}
\def\Top{{\mathbb T}}
\def\Kop{{\mathbb K}}
\def\normal{{\sf N}}
\def\proj{{\mathsf P}}
\def\bbV{{\mathbb V}}
\def\sW{{\mathsf W}}
\def\sM{{\mathsf M}}
\def\T{{\mathbb T}}
\def\K{{\mathbb K}}
\def\H{{\mathbb H}}
\def\Unif{{\sf Unif}}
\def\normal{{\sf N}}
\def\Uop{{\mathbb U}}
\def\Hop{{\mathbb H}}
\def\Sop{{\mathbb S}}
\def\proj{{\mathsf P}}
\def\ik{{\mathsf k}}
\def\il{{\mathsf l}}
\def\sM{{\sf M}}
\def\RKHS{{\sf RKHS}}
\def\RF{{\sf RF}}
\def\NT{{\sf NT}}
\def\NN{{\sf NN}}
\def\reals{{\mathbb R}}
\def\integers{{\mathbb Z}}
\def\naturals{{\mathbb N}}
\def\proj{{\mathsf P}}
\def\Hop{{\mathbb H}}
\def\Uop{{\mathbb U}}

\def\oD{\overline{D}}
\def\ta{\tilde{a}}
\def\tR{\tilde{R}}
\def\ttR{\dbtilde{R}}
\def\tba{\tilde{\boldsymbol a}}
\def\bq{{\boldsymbol q}}

\def\hR{\hat{R}}
\def\Lip{{\rm Lip}}
\def\sL{\mbox{\rm\tiny L}}
\def\sNL{\mbox{\rm\tiny NL}}
\def\seff{\mbox{\rm\tiny eff}}
\def\smix{\mbox{\rm\tiny mix}}
\def\seq{\mbox{\rm\tiny seq}}
\def\slin{\mbox{\rm\tiny lin}}
\def\sTV{\mbox{\rm\tiny TV}}
\def\sGF{\mbox{\rm\tiny GF}}
\def\samp{\mbox{\rm\tiny s}}
\def\wid{\mbox{\rm\tiny w}}
\def\of{\overline{f}}
\def\obtheta{\overline{\boldsymbol \theta}}
\def\stest{\mbox{\tiny\rm test}}

\def\ERM{{\rm ERM}}
\def\Sp{{\mathbb S}}
\def\oalpha{\overline{\alpha}}
\def\hE{\widehat{{\mathbb E}}}
\def\hh{\hat{h}}
\def\tih{\tilde{h}}

\def\oby{\overline{\boldsymbol y}}
\def\br{{\boldsymbol r}}
\def\bfe{{\boldsymbol e}}
\def\bff{{\boldsymbol f}}

\def\oq{\overline{q}}

\def\tlambda{\tilde{\lambda}}

\def\ratio{\zeta}


\usepackage{color}

\newcommand{\am}[1]{\noindent{{\color{red}\textbf{\#\#\# AM:}
\textsf{#1} \#\#\#}}}

\def\cuB{\mathscrsfs{B}}
\def\cuV{\mathscrsfs{V}}

\def\SNR{{\sf SNR}}
\def\rank{{\rm rank}}
\def\hbK{\hat{\boldsymbol K}}
\def\hrho{\widehat{\rho}}

\def\eval{s}
\def\Eval{{\boldsymbol S}}

\def\uF{\underline{F}}
\def\ulambda{\underline{\lambda}}
\def\Risk{{L}}
\def\hRisk{\widehat{L}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\biassquared}{{\textsc{bias}^2}}
\newcommand{\variance}{{\textsc{var}}}
\newcommand{\biassquaredemp}{{\widehat{\textsc{bias}}^2}}
\newcommand{\varianceemp}{{\widehat{\textsc{var}}}}

%\def\deq{\triangleq}
\def\deq{:=}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{\,T}}}} 
\newcommand{\trace}{\mathsf{tr}}
\newcommand{\ind}[1]{\ensuremath{{\mathbf I}{\left\{#1\right\}}}}
\newcommand{\indicator}[1]{\ensuremath{\boldsymbol{1}\left[#1\right]}}
\newcommand{\inner}[1]{\left\langle #1 \right\rangle}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\onehalf}{\ensuremath{\frac{1}{2}}}
\newcommand{\bone}{\ensuremath{\mathbf{1}}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\card}{\mbox{card}}
%\renewcommand{\star}{\text{star}}
\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}} \ }
\newcommand{\argmax}[1]{\underset{#1}{\mathrm{argmax}} \ }
\newcommand{\avgni}{\frac{1}{n}\sum_{i=1}^n}
\newcommand{\avgnt}{\frac{1}{n}\sum_{t=1}^n}

% Expectations and probability
\newcommand{\Ebr}[1]{\mathbb{E}\left\{ #1 \right\}} % curly braces
\newcommand{\En}{\mathbb{E}}  % no brackets or braces
\newcommand{\Es}[2]{\mathbb{E}_{#1}\left[ #2 \right]} % subscript + brackets
\newcommand{\Ps}[2]{\mathbb{P}_{#1}\left[ #2 \right]}
\newcommand{\Prob}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\Eunderone}[1]{\underset{#1}{\E}}
\newcommand{\Eunder}[2]{\underset{\underset{#1}{#2}}{\E}}


% Learning/prediction
\newcommand{\loss}{\mathbf\ell}
\newcommand{\algo}{\widehat{f}}
%\newcommand{\prederm}{\widehat{f}_\text{\tiny erm}}
\newcommand{\prederm}{\widehat{f}_{\scalebox{.4}{erm}}}
\newcommand{\hatf}{\ensuremath{\hat{f}}}
\newcommand{\pred}{\widehat{y}}

% Algebra
%\newcommand\norm[1]{\lVert#1\rVert}

==> preamble.tex <==
% --- inline annotations
%


==> secs/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer:  \answerYes{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations are discussed in the Conclusion Section in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The informal statements are in the main paper Section \ref{sec:method}, and the full formal
 proofs can be found in the Appendix \ref{sec:appendix_proof}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: : The detailed information can be found in Section \ref{sec:experiments}. We also release our code anonymously at \url{https://anonymous.4open.science/r/FedProj_Neurips-63C1}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The code can be found anonymously at \url{https://anonymous.4open.science/r/FedProj_Neurips-63C1}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: The detailed information can be found in Section \ref{sec:experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: We conduct the main experiments in the main paper Section 7 over 3 independent trials with different random seeds and average results with the standard deviation
is reported in Tables \ref{tab:fl_results}, \ref{tab:fl_results_nlp} and \ref{tab:wd_ablation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: The information can be found in Section \ref{subsec:implementation_details} under implementation details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Our research and paper closely follows the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer:  \answerNA{}.
    \item[] Justification: : This paper focuses on advancing technical methodologies in federated learning and does not directly engage with specific societal impacts, as the applications of the proposed method are varied and context-dependent. The societal implications would
    largely depend on the specific use cases implemented by subsequent practitioners.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer:  \answerNA{}.
    \item[] Justification: : This paper primarily focuses on a technical methodological approach without releasing any models. The potential for misuse depends on specific applications by end users, which are beyond the scope of this study.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: The datasets and models used in this work are properly credited in main paper Section \ref{sec:experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}




==> secs/method_2.tex <==

% \section{Methodology}
% In this section, we present \textbf{FedProj}, a novel federated learning framework that mitigates the global knowledge forgetting encountered in standard FedAvg under non-IID settings. Our approach builds upon gradient projection methods from continual learning to constrain local updates and couples this with a server-side knowledge distillation mechanism. We first formalize the federated learning problem and introduce necessary preliminaries, then detail our two-phase method: (1) local training with gradient projection and (2) server-side knowledge distillation.

% \subsection{Problem Formulation and Preliminaries}
% Consider a federated learning system with $N$ clients, where each client $k$ possesses a private dataset $\mathcal{D}_k$ drawn from a non-identically distributed (non-IID) data distribution. The goal is to learn a global model $f(x;\btheta)$ with parameters $\btheta \in \mathbb{R}^d$ by minimizing the weighted aggregate loss:
% \begin{equation}
%     \min_{\btheta} \; \sum_{k=1}^{N} \frac{|\mathcal{D}_k|}{\sum_{j=1}^{N} |\mathcal{D}_j|}\, \mathcal{L}_k(\btheta),
% \end{equation}
% where $\mathcal{L}_k(\btheta)$ is typically a cross-entropy loss defined on the local data at client $k$. In conventional FL methods such as FedAvg, local models are updated independently on heterogeneous data, leading to overfitting on local objectives and loss of global decision boundaries (i.e., \emph{catastrophic forgetting}). To alleviate this, we incorporate two key ideas:
% \begin{enumerate}[label=(\roman*)]
%     \item During local training, in addition to the supervised loss, each client enforces a constraint to preserve global knowledge using a knowledge distillation loss computed on a small public dataset.
%     \item At the server, the aggregated model is further refined via knowledge distillation that integrates the information from all clients.
% \end{enumerate}

% \subsection{Local Training with Gradient Projection}
% At each client, the local objective consists of two components:
% \begin{equation}
%     \mathcal{L}_{\text{local}} = \mathcal{L}_{\text{sup}} + \lambda\, \mathcal{L}_{\text{KD}},
% \end{equation}
% where $\mathcal{L}_{\text{sup}}$ is the supervised loss (e.g., cross-entropy) on the client’s private data, $\mathcal{L}_{\text{KD}}$ is a knowledge distillation loss that measures the discrepancy between the client’s predictions and the global (or teacher) predictions on a public dataset, and $\lambda$ is a balancing coefficient.

% Let $g_{\text{sup}} = \nabla_{\btheta_k}\mathcal{L}_{\text{sup}}$ and $g_{\text{KD}} = \nabla_{\btheta_k}\mathcal{L}_{\text{KD}}$ denote the gradients corresponding to the supervised and distillation losses, respectively. In our setting, while the supervised update drives the model to fit the local objective, it may conflict with the preservation of global knowledge. To counteract this, we impose the constraint that the effective update direction $g$ should not increase the distillation loss, i.e., it should satisfy:
% \begin{equation}
%     \langle g, g_{\text{KD}} \rangle \geq 0.
% \end{equation}
% If $g_{\text{sup}}$ already meets this constraint, no modification is needed. Otherwise, we project $g_{\text{sup}}$ onto the hyperplane defined by $g_{\text{KD}}$. Specifically, the projected gradient is given by:
% \begin{equation}
%     g_{\text{proj}} = g_{\text{sup}} - \frac{\langle g_{\text{sup}}, g_{\text{KD}} \rangle}{\| g_{\text{KD}} \|^2 + \epsilon}\, g_{\text{KD}},
% \end{equation}
% where $\epsilon>0$ is a small constant for numerical stability. The client then updates its parameters via:
% \begin{equation}
%     \btheta_k \gets \btheta_k - \eta\, g_{\text{proj}},
% \end{equation}
% with $\eta$ denoting the local learning rate. This projection step, inspired by methods in continual learning such as Gradient Episodic Memory~\cite{citeturn0file1}, ensures that the local update not only improves performance on the private dataset but also preserves the global decision boundaries encapsulated in the distillation loss.

% \subsection{Server-Side Knowledge Distillation}
% After local training, a subset of clients is sampled and their updated model parameters are sent to the server. The server aggregates these parameters using a weighted averaging scheme (as in FedAvg):
% \begin{equation}
%     \btheta_g = \sum_{k \in S_t} \frac{|\mathcal{D}_k|}{\sum_{j \in S_t} |\mathcal{D}_j|}\, \btheta_k.
% \end{equation}
% In contrast to standard FedAvg, our server also leverages a public dataset $\mathcal{D}_{\text{public}}$ to refine the global model via knowledge distillation. For each sample $\mathbf{x} \in \mathcal{D}_{\text{public}}$, the server computes:
% \begin{itemize}
%     \item \textbf{Teacher logits:} by averaging the predictions of the local models,
%     \begin{equation}
%         \mathcal{Z}_{\text{teacher}} = \frac{1}{|S_t|}\sum_{k \in S_t} f(\mathbf{x}; \btheta_k);
%     \end{equation}
%     \item \textbf{Student logits:} by evaluating the global model,
%     \begin{equation}
%         \mathcal{Z}_{\text{student}} = f(\mathbf{x}; \btheta_g).
%     \end{equation}
% \end{itemize}
% The server-side distillation loss is defined as:
% \begin{equation}
%     \mathcal{L}_{\text{KD}}^{\text{server}} = T^2\, \text{KL}\Big(\sigma\big(\mathcal{Z}_{\text{student}}/T\big) \,\|\, \sigma\big(\mathcal{Z}_{\text{teacher}}/T\big)\Big),
% \end{equation}
% where $T$ is the temperature hyperparameter and $\sigma(\cdot)$ denotes the softmax function. To further stabilize the distillation process, a regularization term is introduced to prevent the global model from deviating too far from the aggregated model:
% \begin{equation}
%     \mathcal{L}_{\text{reg}} = \gamma\, \|\btheta_g - \btheta_g^{(0)}\|^2,
% \end{equation}
% where $\btheta_g^{(0)}$ represents the aggregated model prior to distillation and $\gamma$ is a regularization coefficient. The overall server-side update is performed by minimizing:
% \begin{equation}
%     \mathcal{L}_{\text{server}} = \mathcal{L}_{\text{KD}}^{\text{server}} + \mathcal{L}_{\text{reg}},
% \end{equation}
% using gradient descent with a suitable learning rate.

% \subsection{Discussion}
% This two-stage approach ensures that local training does not conflict with the global knowledge learned across clients, while the server-side refinement leverages ensemble information to further improve generalization. By integrating gradient projection during local updates and a dedicated knowledge distillation step at the server, \textbf{FedProj} effectively mitigates catastrophic forgetting, leading to improved convergence and performance under non-IID conditions.

% Possible reviewer concerns may include the clarity of the constraint derivation, the choice of public dataset for knowledge distillation, and the sensitivity of hyperparameters such as $\lambda$, $\gamma$, and $T$. We address these issues in the experimental section and provide comprehensive ablation studies to validate the robustness of our method.
%

\section{Methodology}
In this section, we introduce \textbf{FedProj}, a novel federated learning algorithm designed to mitigate \textit{catastrophic forgetting} in non-IID settings. Our method integrates \textit{gradient projection} with \textit{global knowledge distillation} (KD) to ensure better knowledge retention and generalization across clients.  

\subsection{Problem Formulation}
Consider a federated learning system with $N$ clients, each possessing a private dataset $\mathcal{D}_k$ drawn from a non-IID distribution. The objective is to train a global model $f_{\btheta}$ by aggregating decentralized updates while preserving global knowledge across heterogeneous client data. Traditional FL methods suffer from local model overfitting, leading to a loss of global knowledge—referred to as \textit{catastrophic forgetting}.  To address this, we propose \textbf{FedProj}, where each client incorporates knowledge distillation and a gradient projection step that ensures local updates align with global knowledge.  

\subsection{Federated Learning with FedProj}

FedProj consists of a \textbf{server-side aggregation} process and a \textbf{client-side update} process, both working in tandem to optimize model learning. 

\subsubsection{Server-Side Training Procedure}

The server in FedProjKD enhances traditional federated learning by integrating knowledge distillation, improving generalization, and mitigating model drift. After aggregating client models using FedAvg, the server refines the global model by leveraging soft logits from clients. 

Unlike standard FedAvg, which directly averages model weights, our approach performs \textbf{logits averaging}, ensuring that the global model learns from client outputs rather than just their parameters. This reduces overfitting to specific client distributions and leads to better convergence. 

Furthermore, global knowledge distillation is applied using a public dataset. The global model is trained to mimic the average client logits, improving its alignment with diverse client knowledge. A regularization term ensures stability and prevents catastrophic forgetting. This additional distillation step makes FedProjKD more robust in heterogeneous environments compared to conventional federated learning. The complete procedure is outlined in Algorithm~\ref{alg:FedProjKD}.

\begin{algorithm}[H]
\caption{Federated Learning with FedProj and Knowledge Distillation}
\label{alg:FedProjKD}
\begin{algorithmic}[1]

\REQUIRE number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epochs ($E$), local batch size ($B$), learning rate ($\eta$), temperature ($T$), distillation learning rate ($\eta_d$), distillation epochs ($E_d$), regularization coefficient ($\gamma$).

\STATE \textbf{Server Executes:}
\STATE Initialize global model $\btheta_g^0$
\FOR {$t = 0, 1, \ldots, T-1$}
    \STATE Sample $m = \max(C \cdot N,1)$ clients $S_t$
    \FOR {$k \in S_t$ \textbf{in parallel}}
        \STATE $\btheta^{t+1}_{k} \gets \mathtt{ClientUpdate}(k; \btheta^t_{g})$
    \ENDFOR

    \STATE \textbf{FedAvg:}  
    \STATE $\btheta^{t+1}_g = \sum_{k \in S_t} \frac{|D_k|}{\sum_{j \in S_t} |D_j|} \btheta^{t+1}_k$

    \STATE \textbf{Logits Averaging:}  
    \STATE $\mathcal{Z}_{\text{teacher}} = \frac{1}{|S_t|} \sum_{k \in S_t} f_k(\mathcal{D}_{\text{public}}; \btheta_k^{t+1})$

    \STATE \textbf{Global Model KD:}
    \FOR {$e = 1, \ldots, E_d$}
        \FOR {each batch $(\mathbf{x}, \mathbf{z}_{\text{teacher}}) \in \mathcal{D}_{\text{public}}$}
            \STATE Compute student logits: \\ \hspace{0.5cm}$\mathcal{Z}_{\text{student}} = f_g(\mathbf{x}; \btheta_g)$
            \STATE Compute losses:
            \STATE $\mathcal{L}_{\text{KD}} = T^2 \cdot \text{KL}(\sigma(\mathcal{Z}_{\text{student}} / T), \sigma(\mathcal{Z}_{\text{teacher}} / T))$
            \STATE $\mathcal{L}_{\text{reg}} = \gamma \sum_{i} \|\btheta_g^{(i)} - \btheta_g^{(i,0)}\|^2$
            \STATE Update model: \\ \hspace{0.5cm}$\btheta_g \gets \btheta_g - \eta_d \nabla_{\btheta_g} (\mathcal{L}_{\text{KD}} + \mathcal{L}_{\text{reg}})$
        \ENDFOR
    \ENDFOR
\ENDFOR

\end{algorithmic}
\end{algorithm}


\subsubsection{Client-Side Training with FedProj}

Each participating client receives the global model parameters $\btheta_g$ and updates them locally for $E$ epochs using its private dataset. Unlike standard federated learning, which can cause client models to drift significantly, FedProj incorporates \textbf{projected gradient updates} to balance local adaptation with global knowledge retention, mitigating catastrophic forgetting and improving generalization.

\paragraph{Supervised Learning}  
For each mini-batch $(\mathbf{x}, \mathbf{y})$ from the private dataset, the client computes logits $\mathcal{Z}_{\text{local}} = f_k(\mathbf{x}; \btheta_k)$ and the supervised loss using cross-entropy:  
\begin{equation}
    \mathcal{L}_{\text{sup}} = \ell(\mathcal{Z}_{\text{local}}, \mathbf{y}).
\end{equation}
This enables clients to learn from their private data while preserving privacy.

\paragraph{Knowledge Distillation}  
To maintain consistency with global knowledge, clients distill knowledge from a public dataset. Given a batch $(\mathbf{x}_t, \mathcal{Z}_{t})$, the client computes student logits $\mathcal{Z}_{\text{student}} = f_k(\mathbf{x}_t; \btheta_k)$ and minimizes the KL-divergence loss:  
\begin{equation}
    \mathcal{L}_{\text{KD}} = T^2 \cdot \text{KL}(\sigma(\mathcal{Z}_{\text{student}} / T), \sigma(\mathcal{Z}_{t} / T)).
\end{equation}
This process prevents client models from deviating too much from the global model, stabilizing convergence.

\paragraph{Projected Gradient Update}  
Instead of naïve gradient updates that may overwrite global knowledge, FedProj applies a projection step. The gradients of both losses are computed as  
$g_{\text{new}} = \nabla_{\btheta_k} \mathcal{L}_{\text{sup}}$ and $g_{\text{glob}} = \nabla_{\btheta_k} \mathcal{L}_{\text{KD}}$.  
To preserve essential global knowledge, the projection removes the conflicting component:  
\begin{equation}
    g_{\text{proj}} = g_{\text{new}} - \frac{\langle g_{\text{new}}, g_{\text{glob}} \rangle}{\| g_{\text{glob}} \|^2 + \epsilon} g_{\text{glob}}.
\end{equation}
where $\epsilon$ ensures numerical stability. This step enhances \textbf{generalization and robustness} while preventing catastrophic forgetting.

\paragraph{Model Update}  
Finally, the model is updated using the projected gradient:  
\begin{equation}
    \btheta_k \gets \btheta_k - \eta g_{\text{proj}}.
\end{equation}
After $E$ epochs, the updated parameters $\btheta_k$ are sent back to the server. This efficient training strategy ensures that FedProj preserves global knowledge while allowing local models to adapt, leading to superior performance in federated settings.



% \subsection{Advantages of FedProjKD}
% The proposed FedProjKD method offers the following key advantages:
% \begin{itemize}
%     \item \textbf{Mitigating Catastrophic Forgetting:} The projected gradient update ensures that client models retain previously learned knowledge while incorporating new updates.
%     \item \textbf{Improved Generalization:} Knowledge distillation from the global model helps clients benefit from shared knowledge without directly sharing data.
%     \item \textbf{Efficient Convergence:} The integration of FedProj with knowledge distillation accelerates convergence by preventing destructive gradient updates.
%     \item \textbf{Privacy Preservation:} Since only model parameters and logits are exchanged, data privacy is maintained while benefiting from global knowledge transfer.
% \end{itemize}

This combined approach ensures that local learning does not interfere with global knowledge, effectively mitigating catastrophic forgetting while improving FL performance.

\begin{algorithm}[H]
\caption{ClientUpdate with FedProj and Knowledge Distillation}
\label{alg:ClientFedProjKD}
\begin{algorithmic}[1]
\REQUIRE Local dataset $\mathcal{D}_k$, learning rate $\eta$, temperature $T$, distillation dataset $\mathcal{D}_{\text{public}}$, regularization $\gamma$.
\STATE Initialize local model $\btheta_k$.
\FOR{$e = 1$ to $E$} 
    \FOR{each mini-batch $(\mathbf{x}, \mathbf{y}) \sim \mathcal{D}_k$} 
        \STATE Compute local logits: $\mathcal{Z}_{\text{local}} = f_k(\mathbf{x}; \btheta_k)$
        \STATE Compute supervised loss: $\mathcal{L}_{\text{sup}} = \ell(\mathcal{Z}_{\text{local}}, \mathbf{y})$
        \STATE Sample public batch: $(\mathbf{x}_t, \mathcal{Z}_{t}) \sim \mathcal{D}_{\text{public}}$
        \STATE Compute student logits: $\mathcal{Z}_{\text{student}} = f_k(\mathbf{x}_t; \btheta_k)$
        \STATE Compute KD loss:\\ \hspace{0.5cm} $\mathcal{L}_{\text{KD}} = T^2 \cdot \text{KL}(\sigma(\mathcal{Z}_{\text{student}} / T), \sigma(\mathcal{Z}_{t} / T))$
        \STATE Compute gradients:\\ \hspace{0.5cm}$g_{\text{new}} = \nabla_{\btheta_k} \mathcal{L}_{\text{sup}}, \quad g_{\text{glob}} = \nabla_{\btheta_k} \mathcal{L}_{\text{KD}}$
        \STATE Compute projected gradient:\\ \hspace{0.5cm}$g_{\text{proj}} = g_{\text{new}} - \frac{\langle g_{\text{new}}, g_{\text{glob}} \rangle}{\| g_{\text{glob}} \|^2 + \epsilon} g_{\text{glob}}$
        \STATE Update model parameters: \\ \hspace{0.5cm} $\btheta_k \gets \btheta_k - \eta g_{\text{proj}}$
    \ENDFOR
\ENDFOR
\STATE \textbf{return} $\btheta_k$
\end{algorithmic}
\end{algorithm}








% new local training technique which 
\subsubsection*{Step 1: Ensemble Knowledge Transfer}

\begin{align}
    \mathcal{L} = & \ \text{KL} \left(\sigma\left(\frac{1}{K} \sum_k f_k(x; w_k) \right), \sigma(f_g(x; w_g)) \right) \notag \\
    & + \lambda \norm{W_g - W_{avg}}^2 + \gamma \norm{F_g - F_{avg}}^2
\end{align}

% \begin{algorithm}
% \caption{FedProj: Federated Learning with Projection-based Knowledge Distillation}
% \label{alg:FedProj}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Number of rounds $T$, clients $K$, local epochs $E$, learning rate $\eta$, projection function $P$, distillation temperature $T_d$, distillation steps $S_d$, regularization weight $\gamma$
% \State \textbf{Initialize:} Global model $w^0$
% \For{$t = 1$ to $T$}
%     \State Sample a subset of clients $\mathcal{S}_t$
%     \For{each client $k \in \mathcal{S}_t$ \textbf{in parallel}}
%         \State $w_k^t \gets w^{t-1}$ \Comment{Initialize with global model}
%         \For{local epoch $e = 1$ to $E$}
%             \State Update $w_k^t$ using local data
%             \State $w_k^t \gets P(w_k^t)$ \Comment{Apply projection}
%         \EndFor
%         \State Send updated model $w_k^t$ to server
%     \EndFor
%     \State Compute aggregation weights $\alpha_k = \frac{n_k}{\sum_{i \in \mathcal{S}_t} n_i}$
%     \State Aggregate models: $w^t \gets \sum_{k \in \mathcal{S}_t} \alpha_k w_k^t$
    
%     \Comment{\textbf{Logits Aggregation}}
%     \State Collect logits $\mathcal{L}_k$ from each client $k \in \mathcal{S}_t$ on public dataset
%     \State Compute teacher logits: $\mathcal{L}_T \gets \frac{1}{|\mathcal{S}_t|} \sum_{k \in \mathcal{S}_t} \mathcal{L}_k$
%     \State Store $\mathcal{L}_T$ in public dataset

%     \Comment{\textbf{Global Knowledge Distillation}}
%     \State Load $w^t$ into global model
%     \For{distillation step $s = 1$ to $S_d$}
%         \State Sample batch $(x, y, \mathcal{L}_T)$ from public dataset
%         \State Compute student logits: $\mathcal{L}_S \gets f(x; w^t)$
%         \State Compute KL divergence loss:
%         \[
%         \mathcal{L}_{KD} = \text{KLDivLoss}(\text{log\_softmax}(\mathcal{L}_S / T_d), \text{softmax}(\mathcal{L}_T / T_d))
%         \]
%         \State Compute regularization term: 
%         \[
%         \mathcal{R} = \sum_{i} ||w^t_i - w^{t-1}_i||^2
%         \]
%         \State Compute total loss: 
%         \[
%         \mathcal{L} = T_d^2 \mathcal{L}_{KD} + \gamma \mathcal{R}
%         \]
%         \State Update $w^t$ via gradient descent
%     \EndFor
%     \State $w^t \gets P(w^t)$ \Comment{Apply projection}
% \EndFor
% \end{algorithmic}
% \end{algorithm}


